SwarmUS: An open hardware and software on-board platform for swarm robotics development

Real life implementations of distributed swarm robotics are rare. The standardization of a general purpose swarm robotics platform could greatly accelerate swarm robotics towards real life implementations. The SwarmUS platform is an open-source hardware and software on-board embedded system designed to be added onto existing robots while providing them with swarm features, thus proposing a new take on the platform standardization problem. These features include a distributed relative localization system based on Ultra-Wideband, a local communication system based on Wi-Fi and a distributed coordination system based on the Buzz programming language between robots connected within a SwarmUS platform. Additionally, a human-swarm interaction mobile application and an emulation of the platform in the Robot Operating System (ROS) is presented. Finally, an implementation of the system was realized and tested on two types of robots : a TurtleBot3 Burger and two Pioneer 2DX.

==> plan.tex <==
- A ''proposed take of a swarm system''
- Present the needs of robot to join other robots in a swarm
- Le pourquoi avant le quoi
- What was done with SwarmUS


Besoin de du swarm -> besoins techniques de robots pour faire un swarm -> réponse de SwarmUS + description

System validated on 2 pioneer and 1 turtlebot doing a Follow the leader behavior and in a ROS simulation


Interloc works with 3 synchronised UWB radios
Communications take care of with an independant WiFi network
Swarm intelligence made with the integration of Buzz

Add detailed of where each system are explained 2 pages
- Glo - Étienne
		Diagramme global sur la page 1 et section 2 sur la page suivante
- Interloc - Phil - DONE
- Coordination features (+Simulation) - Gab
- Communication features - Gab
- Augmented Reality HMI - Gab
		Très court, potentiellement coupé
- System Integration (dimesions, connexion) - Phil - DONE

Results: 1.5 pages          
- Localization (Precision (r + theta), refresh rate (linked to swarm scale)) - Phil - done
- Coordination - Follow the leader limitation - Gab
- Limitation integaration (sensor pertubations, mecanic inteference, ) - Étienne
- Communication (bandwidth, maximum swarm scale) - Gab
- Hardware (power consumption, cost) - Phil - done


Discussion (ameliorations) 0.5
- Localisation - PHIL - Done
- Hardware - PHIL - Done

Conclusion: 0.5 pages - Étienne
- Sommaire
- Développements futurs
		- V2 hardware (attention, pas faire de promesses)
 - Intégration dans des projets


Acknoledgement: 
- FM, Jon

Abstract:
-

Keywords:
- 

Referecens (0.25 pages)

